Scalable Hierarchical Agglomerative Clustering

The applicability of agglomerative clustering, for inferring both hierarchical and flat clustering, is limited by its scalability. Existing scalable hierarchical clustering methods sacrifice quality for speed and often lead to over-merging of clusters. In this paper, we present a scalable, agglomerative method for hierarchical clustering that does not sacrifice quality and scales to billions of data points. We perform a detailed theoretical analysis, showing that under mild separability conditions our algorithm can not only recover the optimal flat partition, but also provide a two-approximation to non-parametric DP-Means objective. This introduces a novel application of hierarchical clustering as an approximation algorithm for the non-parametric clustering objective. We additionally relate our algorithm to the classic hierarchical agglomerative clustering method. We perform extensive empirical experiments in both hierarchical and flat clustering settings and show that our proposed approach achieves state-of-the-art results on publicly available clustering benchmarks. Finally, we demonstrate our method's scalability by applying it to a dataset of 30 billion queries. Human evaluation of the discovered clusters show that our method finds better quality of clusters than the current state-of-the-art.

==> zz_fig_hac_alg.tex <==
\begin{algorithm}
\caption{Hierarchical Agglomerative Clustering}\label{alg:hac}
\begin{algorithmic}[1]
\Function{HAC}{$\dataset$ : Dataset , $f$: Linkage}
\State $\mathcal{T} \leftarrow \ \{ \{x_1\}, \dots, \{x_N\} \} $ 
\While {$|\mathcal{T}| > 1$}
\State $C_1,C_2 \leftarrow \argmin_{C \neq C' \in \mathcal{V}} f(C,C')$
\State $C \leftarrow C_1 \cup C_2$ 
\State $\mathcal{T} \leftarrow \mathcal{T} \setminus \{C_1\}$
\State $\mathcal{T} \leftarrow \mathcal{T} \setminus \{C_2\}$
\State $\mathcal{T} \leftarrow \mathcal{T}  \cup \{C\}$
\EndWhile
\State \textbf{return} $\mathcal{T}$
\EndFunction
\end{algorithmic}
\end{algorithm}



==> zz_fig_rounds_plot.tex <==
\begin{figure*}
    \centering%
    \includegraphics[width=0.23\textwidth]{zzz_fig_rounds_cost.pdf}
    \includegraphics[width=0.23\textwidth]{zzz_fig_rounds_time.pdf}
    \includegraphics[width=0.23\textwidth]{zzz_fig_rounds_f1.pdf}
    \includegraphics[width=0.23\textwidth]{zzzz_fig_ablation_Speaker_numcls.pdf}
    \vspace{-3mm}
    \caption{\textbf{Number of Rounds} The impact on number of rounds $(L)$ in \scc algorithm, on DP-mean cost, running time, F1, and number of clusters on Speaker dataset. For DP-means and F1, we report for $\lambda = \{ 1.5, 2\}$.}
    \label{fig:rounds}\vspace{-3mm}
\end{figure*}
